Two Views, One Fix: Multi-Modal Learning for Automated Vulnerability Repair

Many vulnerabilities require edits in non-contiguous code regions that are connected by control- and data-flow dependencies. Token sequences represent these dependencies poorly. In a comparison of 24 source-level approaches, those that use code structure serialize it into tokens, use it to guide attention, or use it to select prompt content. None passes the graph itself to the repair model. We present GraphT5, a graph-augmented Transformer for Automated Vulnerability Repair. GraphT5 reads two views of a vulnerable function: its source code and a Vulnerability Dependence Graph (VDG), a slice of the Code Property Graph that keeps the dependencies relevant to repair. A CodeT5-initialized text encoder and a VDG encoder feed a decoder with gated dual cross-attention. We evaluate GraphT5 on 2,411 C/C++ test samples from three datasets. It outperforms VulMaster by an average relative improvement of 17.1% in Exact Match, 19.6% in BLEU-4, and 8.1% in CodeBLEU, and exceeds zero-shot GPT-4o and Gemini 2.5 Pro in static similarity on two datasets. Under dynamic validation, GraphT5 produces plausible patches for 12 of 81 Vul4C vulnerabilities, tied with the best baseline, and test-passing patches for 15 of 35 Vul4J cases, the third-highest reported total.

==> acronyms.tex <==
\DeclareAcronym{avr}{
	short = AVR,
	long = Automated Vulnerability Repair
}

\DeclareAcronym{avd}{
	short = AVD,
	long = Automatic Vulnerability Detection
}

\DeclareAcronym{apr}{
	short = APR,
	long = Automatic Program Repair
}

\DeclareAcronym{rv}{
	short = RV,
	long = Recurrent Vulnerability,
	long-plural-form = Recurrent Vulnerabilities
}

\DeclareAcronym{esc}{
	short = ESC,
	long = Eliminate Suspicious Commit,
}

\DeclareAcronym{cwe}{
	short = CWE,
	long = Common Weakness Enumeration
}

\DeclareAcronym{cve}{
	short = CVE,
	long = Common Vulnerabilities and Exposures,
	long-plural-form = Common Vulnerabilities and Exposures
}

\DeclareAcronym{cvss}{
	short = CVSS,
	long = Common Vulnerability Scoring System
}

\DeclareAcronym{sbt}{
	short = SBT,
	long = Structure-based Traversal
}

\DeclareAcronym{llm}{
	short = LLM,
	long = Large Language Model
}

\DeclareAcronym{pov}{
	short = PoV,
	long = Proof-of-Vulnerability,
	long-plural-form = Proof-of-Vulnerabilities
}

\DeclareAcronym{poc}{
	short = PoC,
	long = Proof-of-Concept,
	long-plural-form = Proof-of-Concept
}

\DeclareAcronym{vcc}{
	short = VCC,
	long = Vulnerability-Contributing Commit,
}

\DeclareAcronym{ebnf}{
	short = EBNF,
	long = Extended Backus-Naur form
}

\DeclareAcronym{rnn}{
	short = RNN,
	long = Recurrent Neural Network
}

\DeclareAcronym{lstm}{
	short = LSTM,
	long = Long Short-Term Memory
}

\DeclareAcronym{gtn}{
	short = GTN,
	long = Graph Transformer Network
}

\DeclareAcronym{fid}{
	short = FiD,
	long = Fusion-in-Decoder
}

\DeclareAcronym{s2s}{
	short = seq2seq,
	long = sequence-to-sequence
}

\DeclareAcronym{bpe}{
	short = BPE,
	long = byte-pair encoding
}

\DeclareAcronym{dca}{
	short = DCA,
	long = dual cross-attention
}

\DeclareAcronym{rms}{
	short = RMS,
	long = root mean square
}
\DeclareAcronym{ast}{
	short = AST,
	long = Abstract Syntax Tree
}

\DeclareAcronym{cpg}{
	short = CPG,
	long = Code Property Graph,
}

\DeclareAcronym{coi}{
	short = CoI,
	long = Code of Interest
}

\DeclareAcronym{ncs}{
	short = NCS,
	long = Natural Code Sequence
}

\DeclareAcronym{vdg}{
	short = VDG,
	long = Vulnerability Dependence Graph,
}

\DeclareAcronym{cfg}{
	short = CFG,
	long = Control Flow Graph,
}

\DeclareAcronym{dfg}{
	short = DFG,
	long = Data Flow Graph,
}

\DeclareAcronym{pdg}{
	short = PDG,
	long = Program Dependence Graph,
}

\DeclareAcronym{sdg}{
	short = SDG,
	long = System Dependence Graph
}

\DeclareAcronym{met}{
	short = MET,
	long = Minimum Edit Tree
}

\DeclareAcronym{sbtm}{
	short = SBTM,
	long = Structure-based Traversal for Edge-Labeled Multigraphs
}

\DeclareAcronym{gnn}{
	short = GNN,
	long = Graph Neural Network,
}

\DeclareAcronym{ggnn}{
	short = GGNN,
	long = Gated Graph Neural Network
}

\DeclareAcronym{gat}{
	short = GAT,
	long = Graph Attention Network
}

\DeclareAcronym{t5}{
	short = T5,
	long = Text-to-Text Transfer Transformer,
}


==> figures/background/modification/patched_code.tex <==
\begin{minipage}{13.5cm}
    \begin{diffbox}[nobeforeafter]{Patched Code}
        \begin{minted}[ 
      fontsize=\small,
      linenos=true,
      breaklines,
      numbersep=5pt,
      xrightmargin=0pt,
      frame=none,
      framesep=2mm,
      baselinestretch=1.2,
      fontfamily=tt,
      highlightlines={1-3}, 
      highlightcolor=diffadd,
      escapeinside=||
  ]{java}
|\texttt{+}| public byte[] getSalt() {
|\texttt{+}|    byte[] salt = new byte[this.saltLength];
|\texttt{+}|    sr.nextBytes(salt);
     return salt;
 }
    \end{minted}
    \end{diffbox}
\end{minipage}


==> figures/background/modification/vulnerable_code.tex <==

\begin{minipage}{13.5cm}
    \begin{diffbox}[nobeforeafter]{Vulnerable Code}
        \begin{minted}[
      fontsize=\small,
      linenos=true,
      breaklines,
      numbersep=5pt,
      xrightmargin=0pt,
      frame=none,
      framesep=2mm,
      baselinestretch=1.2,
      fontfamily=tt,
      highlightlines={1,2}, 
      highlightcolor=diffdelete, 
      numberblanklines=false,
      escapeinside=||
      ]{java}
|\texttt{-}| public byte[] getSalt() throws NoSuchAlgorithmException {
|\texttt{-}|   byte[] salt = RandomUtil.randomBytes(this.saltLength);

    return salt;
 }
    \end{minted}
    \end{diffbox}
\end{minipage}

